The $D_s$, $D^+$, $B_s$ and $B$ decay constants from $2+1$ flavor lattice QCD

We present a study of the $D$ and $B$ leptonic decay constants on the MILC $N_f=2+1$ asqtad gauge ensembles using asqtad-improved staggered light quarks and clover heavy quarks in the Fermilab interpretation. Our previous analysis \cite{Bazavov:2011aa} computed the decay constants at lattice spacings $a \approx 0.14, 0.11$ and $0.083$ fm. We have extended the simulations to finer $a \approx 0.058$ and $0.043$ fm lattice spacings, and have also increased statistics; this allows us to address many important sources of uncertainty. Technical advances include a two-step two-point fit procedure, better tuning of the heavy quark masses and a better determination of the axial-vector current matching. The present analysis remains blinded, so here we focus on the improvements and their predicted impact on the error budget compared to the prior analysis.

==> Makefile <==
MAKEFILE= Makefile

VPATH=.:R:figures:chiral

R= R
LATEX= pdflatex
BIBTEX= bibtex

BASE= lat2013-394-fDfB

TEXMAIN= $(BASE).tex
PDFDOC= $(BASE).pdf

TEXSRC= \
  macros.tex \


RPLOTS= \
  R/errorBudget_combined.pdf \


FIGS= \
 PoSlogo.pdf \
 fit-D-Ethan-plotFit-2-col.pdf fit-D-Ethan-plotFit-3-col.pdf fit-D-Ethan-plotExtrapolation.pdf \
 fit-B-Ethan-plotFit-2-col.pdf fit-B-Ethan-plotFit-3-col.pdf fit-B-Ethan-plotExtrapolation.pdf \


BIBS= bib/fDfB.bib

AUX= $(BASE).aux
BIBLIO= $(BASE).bbl

LOGS= $(BASE).aux $(BASE).bbl $(BASE).blg $(BASE).log

$(PDFDOC): $(TEXMAIN) $(FIGS) $(RPLOTS)  $(BIBS) $(BIBLIO) $(MAKEFILE)
	$(LATEX) $(TEXMAIN) && $(LATEX) $(TEXMAIN)


$(BIBLIO) $(AUX): $(TEXMAIN) $(FIGS) $(BIBS) $(MAKEFILE)
	$(LATEX) $(TEXMAIN) && $(BIBTEX) $(BASE)

clean:
	@/bin/rm -f $(LOGS)

preview: $(PDFDOC)
	open /Applications/Preview.app $(PDFDOC)

reader: $(PDFDOC)
	acroread $(PDFDOC) &

# weave to produce .tex
%.tex: %.Rnw
	$(R) CMD Sweave $<

# tangle to extract .R code
%.R: %.Rnw
	$(R) CMD Stangle $<

# generate R plots
%.pdf: %.R
	( d=`dirname $<`; cd $$d ; $(R) CMD BATCH `basename $<` )

errorBudget_arXiv1112p3051.pdf: errorBudget_arXiv1112p3051.dat
errorBudget_combined.pdf: errorBudget_arXiv1112p3051.dat errorBudget_projected.dat
errorBudget_projected.pdf: errorBudget_projected.dat

